LineCounter: Learning Handwritten Text Line Segmentation by Counting

Handwritten Text Line Segmentation (HTLS) is a low-level but important task for many higher-level document processing tasks like handwritten text recognition. It is often formulated in terms of semantic segmentation or object detection in deep learning. However, both formulations have serious shortcomings. The former requires heavy post-processing of splitting/merging adjacent segments, while the latter may fail on dense or curved texts. In this paper, we propose a novel Line Counting formulation for HTLS -- that involves counting the number of text lines from the top at every pixel location. This formulation helps learn an end-to-end HTLS solution that directly predicts per-pixel line number for a given document image. Furthermore, we propose a deep neural network (DNN) model LineCounter to perform HTLS through the Line Counting formulation. Our extensive experiments on the three public datasets (ICDAR2013-HSC, HIT-MW, and VML-AHTE) demonstrate that LineCounter outperforms state-of-the-art HTLS approaches. Source code is available at https://github.com/Leedeng/Line-Counter.

==> 3_Experiment.tex <==
\subsection{Overview}
As one may notice, not all DNNs can work compatibly with the \textit{Line Counting} formulation. For example, a typical convolutional neural network (CNN) will predict the same line number for two disjoint but identical local patches. In the context of \textit{Line Counting}, identical local patches can be of different line numbers. Hence, we need to design a compatible DNN for the \textit{Line Counting} formulation.  

Fig.~\ref{fig.structure} shows the proposed \texttt{LineCounter} network, which is a variant of the classic encoder-decoder network[ref] with three main modules, namely \texttt{Encoder}, \texttt{Counter}, and \texttt{Decoder}. \texttt{Encoder} and \texttt{Decoder} are both CNNs and are symmetric of each other. \texttt{LineCounter} is placed in between of \texttt{Encoder} and \texttt{Decoder} to fulfill the goal of line information propagation along both horizontal and vertical directions by using recurrent sequence learning. Consequently, \texttt{LineCounter} can directly predict the line counting map $C$ from an input document image $D$. 

In the rest of the subsections, we first introduce common settings used in later studies and discuss the ablation study related to each module design. More precisely, we explore the backbone network for both \texttt{Encoder} and \texttt{Decoder}, the topology of recurrent sequence learning for \texttt{Counter}, and finally the importance of enforcing the monotonic property for the \textit{Line Counting} formulation. 



\clearpage


